Probabilistic Stable Functions on Discrete Cones are Power Series (long version)

We study the category Cstabm of measurable cones and measurable stable functions, which is a denotational model of an higher-order language with continuous probabilities and full recursion. We look at Cstabm as a model for discrete probabilities, by showing the existence of a cartesian closed, full and faithful functor which embeds probabilistic coherence spaces (a fully abstract denotational model of an higher-order language with full recursion and discrete probabilities) into Cstabm. The proof is based on a generalization of Bernstein's theorem from real analysis allowing to see stable functions between discrete cones as generalized power series.

==> macros.tex <==
\usepackage{color}
\usepackage{bussproofs}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{stmaryrd}
\RequirePackage{ifthen}
\newcommand{\typeof}{1}
\newcommand{\longv}[1]{\ifthenelse{\equal{\typeof}{0}}{}{#1}}
\newcommand{\shortv}[1]{\ifthenelse{\equal{\typeof}{0}}{#1}{}}
%\newcommand{\remarque}[1]{\textcolor{blue}{#1}}
\newcommand{\remarque}[1]{}
\newcommand{\hide}[1]{}


%% Maths
\newcommand{\NN}{\mathbb{N}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\Rp}[1]{\mathbb{R}_+^{#1}}
\newcommand{\scal}[2]{\langle #1,#2 \rangle}
\newcommand{\mfin}[1]{M_f(#1)}
\newcommand{\mfink}[2]{M_f^{#1}(#2)}
\newcommand{\supp}[1]{\text{Supp}(#1)}
\newcommand{\bnf}{::=}
\newcommand{\midd}{\; \; \mbox{\Large{$\mid$}}\;\;}
\newcommand{\card}[1]{\text{card}(#1)}
\newcommand{\permu}[2]{S_{#1}^{#2}}
\newcommand{\dirac}[1]{\{#1 \}^1}

%% Semantics
\newcommand{\sem}[1]{\llbracket #1 \rrbracket}
\newcommand{\semm}[1]{\llbracket #1 \rrbracket_{\cstabm}}
%%% Category
\newcommand{\pcoh}{\mathbf{Pcoh}}
\newcommand{\kpcoh}{\mathbf{PCoh_!}}
\newcommand{\cstabm}{\mathbf{Cstab_m}}
\newcommand{\cstab}{\mathbf{Cstab}}
\newcommand{\discr}{\mathbf{D}}
\newcommand{\discrm}{\mathbf{D_m}}
\newcommand{\functor}{\mathcal F}
\newcommand{\functorm}{\mathcal F^m}
\newcommand{\functord}{\mathcal G}
\newcommand{\forgetful}{\texttt{Forget}}
%%% Languages
\newcommand{\pcf}{\textsf{PCF}}
\newcommand{\ppcf}{PPCF}

%% Terms
\newcommand{\variables}{\textbf{V}}
\newcommand{\varone}{x}
\newcommand{\vartwo}{y}
\newcommand{\varthree}{z}
\newcommand{\termone}{M}
\newcommand{\termtwo}{N}
\newcommand{\termthree}{L}
\newcommand{\termfour}{K}
\newcommand{\termfive}{T}
\newcommand{\termsix}{U}
\newcommand{\termseven}{P}
\newcommand{\termeight}{Q}

%%% PCS
\newcommand{\pcsone}{X}
\newcommand{\pcstwo}{Y}
\newcommand{\pcsthree}{Z}
\newcommand{\web}[1]{\lvert #1 \rvert}
\newcommand{\prog}[1]{P #1}
\newcommand{\dual}[1]{{(#1)^{\bot}}}


\newcommand{\ttrue}{\textbf{t}}
\newcommand{\ffalse}{\textbf{f}}
\newcommand{\Bool}{\textbf{Bool}}
\newcommand{\unit}{\mathbf{1}}
\newcommand{\arrow}{\multimap}

%% Morphisms in PCoh!
\newcommand{\mapm}[1]{\widetilde{#1}}
\newcommand{\bang}[1]{{!#1}}

%% Cones
\newcommand{\coneone}{C}
\newcommand{\conetwo}{D}
\newcommand{\coneonem}{\overline{C}}
\newcommand{\conetwom}{\overline{D}}
\newcommand{\norm}[2]{ {\| #2 \|}_{#1}}
\newcommand{\pcstocone}[1]{C_{#1}}
\newcommand{\pcstoconem}[1]{\overline{C}_{#1}}
\newcommand{\order}[1]{ \, \preceq_{#1} \,}
\newcommand{\boule}[1]{\mathscr{B} #1}
\newcommand{\bouleopen}[1]{\mathscr{B}^\circ #1}
\newcommand{\openboule}[1]{\bouleopen{#1}}
\newcommand{\partit}[2]{#1 \sim #2}
\newcommand{\parts}[1]{\mathcal P (#1)}
\newcommand{\meastests}[2]{\mathcal{M}^{#2}(#1)}
\newcommand{\meas}[1]{\text{Meas}(#1)}
\newcommand{\measm}[1]{\overline{\text{Meas}(#1)}}
\newcommand{\trmeas}[2]{#1 \rhd #2}
\newcommand{\pathone}{\gamma}

%%Stable Functions
\newcommand{\diff}[2]{\Delta^{#2}_{#1}}
\newcommand{\parteps}[2]{\mathcal P _{#1}(#2)}
\newcommand{\ders}[2]{\mathbf{D}^{#1}{#2}}

%% Fullness result
\newcommand{\morph}[1]{\underline{#1}}

%% DIstributions
\newcommand{\distrs}[1]{\Delta(#1)}

\newcommand{\pathes}[2]{\text{Paths}^{#2}(#1)}

%% Terms

\newcommand{\wfjt}[3]{#1 \vdash #2 \,:\, #3}
\newcommand{\tarr}[2]{#1 \rightarrow #2}
\newcommand{\hole}{[\,]}

%% Types
\newcommand{\typone}{\sigma}
\newcommand{\typtwo}{\tau}
\newcommand{\contone}{\Gamma}
\newcommand{\conttwo}{\Delta}

%%% Family
\newcommand{\fone}{\mathscr{I}}



%%% THEOREMS %%%
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{corollary}{Corollary}
\newtheorem{note}{Note}
\newtheorem{remark}{Remark}
\newenvironment{proof}{\begin{trivlist}
       \item[\hskip \labelsep {\bfseries Proof.}]}{\hfill $\Box$ \end{trivlist}}



